Data-Efficient Symbolic Regression via Foundation Model Distillation

Discovering interpretable mathematical equations from observed data (a.k.a. equation discovery or symbolic regression) is a cornerstone of scientific discovery, enabling transparent modeling of physical, biological, and economic systems. While foundation models pre-trained on large-scale equation datasets offer a promising starting point, they often suffer from negative transfer and poor generalization when applied to small, domain-specific datasets. In this paper, we introduce EQUATE (Equation Generation via QUality-Aligned Transfer Embeddings), a data-efficient fine-tuning framework that adapts foundation models for symbolic equation discovery in low-data regimes via distillation. EQUATE combines symbolic-numeric alignment with evaluator-guided embedding optimization, enabling a principled embedding-search-generation paradigm. Our approach reformulates discrete equation search as a continuous optimization task in a shared embedding space, guided by data-equation fitness and simplicity. Experiments across three standard public benchmarks (Feynman, Strogatz, and black-box datasets) demonstrate that EQUATE consistently outperforms state-of-the-art baselines in both accuracy and robustness, while preserving low complexity and fast inference. These results highlight EQUATE as a practical and generalizable solution for data-efficient symbolic regression in foundation model distillation settings.

==> main_content/introduction-Wangyang.tex <==
\section{Introduction}


Data to equation identifies the optimal function that fits observed values by exploring mathematical expression space. Unlike other data modeling approaches, it does not assume a predefined functional form, offers interpretable equations, and provides clear physical insights for data-driven decision-making tasks. 
Data-to-equation methods have significant applications across various domains, for instance, it is used to discover physical laws, optimize industrial designs, analyze economic causal relationships, extract biological mechanisms from genomic data, etc~\cite{wang2019symbolic,angelis2023artificial,cranmer2020discovering,can2011comparison,claveria2017assessment,la2023flexible}. These methods can model complex systems, support automated scientific discovery, and ensure strong model interpretability.

Foundation models have emerged as powerful tools in data-driven decision-making tasks. By leveraging large-scale pre-training, these models can capture latent patterns across diverse datasets and offer remarkable generalization and adaptability to various tasks. Their ability to discover equations from data further underscores the potential to advance data-to-equation tasks.~\cite{biggio2021neural,kamienny2022end,shojaee2023transformer,holt2023deep,valipour2021symbolicgpt}. 
% genetic programming (GP)~\cite{GP,GP2,GP3,GP6,GP7} iteratively optimizes equations by performing genetic operations such as crossover and mutation on initial expressions. GP algorithms exhibit good performance but suffer from high search complexity, sensitivity to hyperparameters, low computational efficiency, and local optima. Deep learning-based SR~\cite{petersen2019deep,kim2020integration,zhang2023deep,d2022deep} algorithms improve the equations discovery, but these methods train a separate model for each problem and often perform poorly on limited datasets. 
However, there are some limitations:
\ul{1) Limited adaptability to domain-specific datasets.} Without adapting to the unique characteristics of specific domains, foundation models struggle to capture unique patterns within the data. Therefore, the generated equations may fail to achieve the optimal performance.
\ul{2) Mismatch between data and equation patterns.} Transformer-based models regard the data-to-equation task as a language translation problem, which employs an encoder-decoder structure to encode observed data values into embeddings and autoregressively generate the sequence representation of equations via the decoder. These approaches fail to fully consider the differences in patterns between input and output data. As a result, it's difficult to capture latent symbolic information of mathematical expressions, thereby limiting model performance. 
\ul{3) Misaligned data-to-equation objectives.} The training objectives of transformer-based methods are typically borrowed from supervised pre-training in text generation (e.g., token-level cross-entropy loss), which may result in equations with high token-level similarity. However, this does not align optimally with the desired data-to-equation goals such as fitting accuracy and simplicity.

\textbf{Our perspective: Transferring foundation models' numerical pattern recognition, incorporating symbolic knowledge, and optimizing domain-specific embedding spaces for data-to-equation tasks.} We design a fine-tuning framework to transfer knowledge to specific domains, infuse mathematical expressions into the framework to bridge the gap between numerical inputs and symbolic outputs, and adopt optimization strategies in the embedding space tailored to the core goals of data-to-equation. Specifically, 
\ul{1) fine-tuning the foundation model:} We sample a domain-specific dataset and perform targeted fine-tuning to adapt the foundation model for domain-specific tasks. By fine-tuning the model on data that reflects the unique patterns of the target domain, we enable it to generate equations that are aligned with the underlying domain-specific relationships.
\ul{2) infusing symbolic knowledge into the data-to-equation model:} Data-to-equation tasks require mapping numerical inputs into interpretable symbolic equations, but this mapping often overlooks the fundamental differences between these two modalities. By embedding prior knowledge into the model, we introduce a structure-aware perspective that allows the model to capture latent patterns of equations and align them with the underlying information of the numerical data. This approach not only improves interpretability but also facilitates generalization across tasks requiring a deeper understanding of mathematical relationships.
\ul{3) Embedding space optimization for data-to-equation goals:} Traditional training objectives of transformer-based models, such as token-level cross-entropy loss, fail to align with the goal of data-to-equation. By shifting optimization to the embedding space, we directly align the model's search process with these goals, which enables efficient identification of equations that achieve an optimal balance between fitting accuracy and simplicity. This paradigm shift frees the model from the constraints of token-level similarity, and can better handle complex or noisy datasets while maintaining robust performance. 

\textbf{Summary of technical solution.} Inspired by these findings, we propose a fine-tuning framework that incorporates symbolic reasoning and performs a targeted search within the embedding space of the trained model to identify equations that align closely with the desired objectives. To achieve this, we integrate numerical and symbolic knowledge through a dual-encoder system implemented by transformers and LSTM, respectively. This framework fuses numerical embeddings with symbolic embeddings to enhance the model's ability to understand mathematical semantics and facilitate the generation of more accurate equations. Additionally, we design an evaluation metric to measure the fitness between the fusion embeddings and the true equations that we aim to generate, and then employ an evaluator to evaluate it in the latent space. This evaluator provides gradients to guide the search for improved fusion embeddings that balance fitting accuracy and simplicity of generated equations. This approach ensures that the generated equations accurately capture the observed data-label relationships, thereby enhancing the overall performance of SR tasks.

\textbf{Summary of our contributions.}
\ul{1) Fine-tuning Framework.} We propose a principal fine-tuning framework that transfers pre-trained knowledge of data-to-equation foundation models to specific domain
\ul{2) Symbolic Knowledge Integration:} We embed mathematical expressions as prior knowledge, bridging the gap between numerical inputs and symbolic outputs to improve generation performance.
\ul{3) Embedding Space Optimization:} We align the model's generation with data-to-equation goals, such as fitting accuracy and simplicity, through optimization in the embedding space, which enables robust performance.


==> main_content/method-Wangyang.tex <==
\section{The Knowledge Transfer for Task-specific Model Learning}
% 1. overall: finetune dataset -> numerical encoder -> symbolic encoder -> feature fusion -> decoder and train loss


\subsection{Overall Structure}
Figure \textbf{X} presents the overall structure of our method, which integrates symbolic knowledge and latent space optimization to enhance SR tasks. By combining structured symbolic priors with numerical observations and leveraging optimization in the latent space, our approach achieves improved performance in downstream tasks. The method consists of three key components:
1) Offline Asynchronous Data Generator: To construct task-specific datasets for fine-tuning, we employ an offline asynchronous data generator that produces high-quality SR data.
2) Transformer-Based SR Model: The transformer-based SR model jointly processes observed data points, labels, and symbolic equations. Through its encoding and decoding stages, the model leverages both numerical observations and symbolic priors to autoregressively reconstruct more accurate equations.
3) Latent Space Optimization: To refine the generated equations, latent space optimization identifies optimal symbolic embeddings that align with the relationships in the testing dataset. By optimizing the embeddings, this step enhances the model's ability to generate equations that accurately capture the observed data-label relationship.

\subsection{Offline Asynchronous Data Generation}
Symbolic knowledge provides a structured and interpretable representation of the underlying relationships in data, which is particularly valuable for downstream tasks. We developed an offline asynchronous data generator, designed to operate independently of the training process. Our asynchronous generator achieves this by decoupling the data generation process from the training pipeline, allowing the computationally expensive task of equation generation to be handled offline without affecting real-time performance. The data generation process involves the following steps:

\noindent\textbf{Step 1: Sampling Observations.} We sample a observations $(\mathbf{X}, y)$ from a domain-specific dataset such as Feynman dataset.

\noindent\textbf{Step 2: Generating Symbolic Equations.} We use a pre-trained symbolic regression baseline to generate an equation $\Tilde{f}$ that captures the underlying relationships in the sampled observations.

\noindent\textbf{Step 3: Computing Pseudo-Labels.} For the generated equation $\Tilde{f}$, we compute a pseudo-label $\Tilde{y}$ based on the sampled $\mathbf{X}$. This pseudo-label serves as an approximation of the true label $y$.

\noindent\textbf{Step 4: Constructing Data Quadruples.} The resulting data is organized into quadruples $(\mathbf{X}, y, \Tilde{f}, \Tilde{y})$, where $\Tilde{f}$ serves as prior symbolic knowledge, $(\mathbf{X}, \Tilde{y}, \Tilde{f})$ is used to fine-tune the model, and $(y, \Tilde{y})$ is used to evaluate the distinctiveness between the generated and true equations.

We iteratively process these steps in an offline system and finally generate the fine-tuning dataset $(\mathbf{X}_i, y_i, \Tilde{f}_i, \Tilde{y}_i)_{i=1}^n$, where $n$ is the number of training samples.

\subsection{Symbolic Regression Model}
We incorporate symbolic prior knowledge into transformer-based SR models. To achieve this, we developed a dual-encoder system that simultaneously encodes numerical observations and symbolic prior knowledge. This dual-encoding mechanism captures both the numerical relationships in the data and the mathematical semantics of equations, which facilitates the model's ability to learn symbolic patterns and improves the accuracy of generated equations.
The dual-encoder system constructs a latent space, where each vector represents the quality of the generated equations. By manipulating these embedding vectors, we can effectively guide the model toward generating more accurate equations. We designed an evaluation metric to measure the accuracy between the latent embedding and the true target. This metric, combined with a search algorithm, enables the identification of the "optimal point" or "optimal latent vector" in the latent space. The decoder then utilizes this optimized latent representation to generate high-quality equations that align more closely with the desired target.

\noindent\textbf{Numerical Encoder.} We utilize the pre-trained encoder from the backbone~\cite{kamienny2022end} as our numerical encoder. This encoder embeds each sample in the numerical data into a token, which is then processed by a transformer to encode the token sequence into a fixed-length vector. Formally, given a numerical observation $(\mathbf{X}, \Tilde{y})$, where $\Tilde{y}$ is the pseudo label calculated by the generated function $\Tilde{f}$. The numerical encoder outputs a numerical embedding: $E_n = \mathcal{N}(\mathbf{X}, \Tilde{y})$, where $\mathcal{N}$ is the function notation of the numerical encoder.

\noindent\textbf{Symbolic Encoder.} We developed an LSTM-based symbolic encoder that encodes the true function corresponding to the numerical observations as prior symbolic knowledge. Formally, given a generated function $\Tilde{f}$, we follow the rules defined by the pre-trained backbone~\cite{kamienny2022end} to convert $\Tilde{f}$ into a prefix expression, and then tokenize it as $T = (t_1, t_2, ..., t_M)$, where $M$ is the number of tokens. The symbolic encoder outputs a symbolic embedding: $E_s = \mathcal{S}(T)$, where $\mathcal{S}$ is the function notation of the symbolic encoder.

\noindent\textbf{Embedding Fusion.} To effectively combine the information from the the vectors $E_n$ and $E_s$ generated by the two encoders respectively, we employ an attention-based mechanism that aligns $E_s$ to $E_n$. The attention mechanism allows the model to dynamically focus on the most relevant parts of $E_s$ in relation to $E_n$. First, we define the numerical embedding as the query $Q(E_n)$, while the symbolic embedding serves as both the key $K(E_s)$ and the value $V(E_s)$. Second, the attention scores are calculated as the scaled dot product of the query and the transposed key: $scores = Q(E_n)K(E_s)^\top/\sqrt{d_k}$, where $d_k$ is the dimensionality of the embeddings, and scaling by $\sqrt{d_k}$ helps stabilize the gradients during training. Then the attention scores are normalized by the softmax function to produce attention weights: $W = softmax(scores)$. Third, the context vector is computed as the weighted sum of the value embeddings: $context = W \cdot V(E_s)$. Finally, we fuse the two vectors with residual connection: $E_f = E
_n + context$. The model dynamically adapts to the relationships between numerical and symbolic features through the attention weights, providing a more informative representation.

\noindent\textbf{Fusion Eembedding Evaluation.} We expect the fusion embedding space to not only represent each input pair but also preserve their utility. Specifically, the embedding vector should capture the accuracy between the pseudo-labels $\Tilde{y}$ calculated by the equation $\Tilde{f}$ and the true labels $y$ provided by the data matrix. To achieve this, we developed an evaluation metric to measure the R2-score between $\Tilde{y}$ and $y$, as well as to assess the complexity of the equation $\Tilde{f}$, denoted as:
\begin{equation}
    r = (1-\frac{\Sigma_{i=1}^n(\Tilde{y}_i-y_i)^2}{\Sigma_{i=1}^n(\Tilde{y}_i-\bar{y})^2}) + \lambda \cdot exp(-\frac{l(\Tilde{f})}{L}),
\end{equation}
where $l$ is the complexity function notation that calculates the length of $f$ in prefix expression, $L$ is the maximum sequence length, $\lambda$ is a hyperparameter to balance the fitting accuracy and complexity, $\bar{y}$ is the average of the true labels.
Subsequently, we introduced a simple MLP following the attention layer to estimate $r$, denoted by: $\mathcal{L}_{est} = MSE(r, MLP(E_f))$, providing gradient information to guide the search for the 'optimal point' in the embedding space.

\noindent\textbf{Decoder and Train.} The decoder is to reconstruct the tokenized eqautation $T=(t_1, t_2, ..., t_M)$. We incorporate the pre-trained decoder from the backbone as the core component of our decoding process. The decoder predicts the token distribution and generates the tokenized equation using the fused embedding $E_f$. During the decoding process, when predicting the token $t_j$, the partially decoded sequence is $[t_1, t_2, ..., t_{j-1}]$. The probability of the $j$-th token is calculated as follows:
\begin{equation}
    P_\mathcal{S}(t_j|E_f, [t_1, t_2, ..., t_{j-1}]) = \frac{exp(m_j)}{\Sigma_M exp(m)},
\end{equation}
where $m_j$ is the $j$-th output of the softmax layer. To optimize the reconstruction, we minimize the negative log-likelihood of generating sequential tokens to minimize the reconstruction loss between the predicted and ground truth tokens:
\begin{equation}
    \mathcal{L}_{rec} = -\Sigma_{j=1}^M log P_\mathcal{S}(t_j|E_f, [t_1, t_2, ..., t_{j-1}]).
\end{equation}
Finally, we trade off the two losses to form a joint training loss: $\mathcal{L} = \alpha \cdot \mathcal{L}_{est} + \beta \cdot \mathcal{L}_{rec}$, where $\alpha$ and $\beta$ are the hyperparameters to balance the influence of the two loss functions. 

\subsection{Latent Space Optimization and Generation}
\textbf{Why optimize the latent space matter?} The latent space preserves key features of prior symbolic and numerical knowledge. By making slight adjustments to the embedding points, the decoder can produce more optimal results. During the prediction phase, since the true equation for the observed data is unknown, we can search within the latent space for the symbolic equation that best matches the test data. This equation serves as prior knowledge to refine the final generated results. 

\noindent\textbf{Search for the optimal symbolic embedding.} In the training phase, we evaluate each data pair using an evaluator, which assesses its accuracy in predicting $\Tilde{y}$ relative to the ground truth $y$ for the target domain, as well as its complexity. During the prediction phase, we optimize the embedding points in the latent space to identify the optimal representation (i.e., the symbolic equation that performs best on the real data). We select the top-k-performance training data $(\mathcal{X}, \Tilde{y}, \Tilde{f})$ as initial points to find better embedding points. Specifically, we replace the pseudo label with the true label $y$, and feed them into the well-trained numerical and symbolic encoders respectively to obtain a fusion embedding $E_f$. Then we use a gradient-ascent method to move the embedding with $\eta$ steps along the direction maximizing the accuracy $r$, denoted as $E_f^+ = E_f + \eta \cdot \frac{\partial{\theta}}{\partial{E_f}}$, where $\theta$ is the function notation of the evaluator.

\noindent\textbf{Generate the optimal equation.} Once we identify the optimized fusion representation $E_f^+$. We feed $E_f^+$ into the well-trained decoder to generate the final token sequence in an autoregressive manner. We iteratively generate the possible tokens until finding the end token (i.e., <EOS>) and transform this token sequence into an equation based on the predefined rules. Finally, we use the Broyden–Fletcher–Goldfarb–Shanno algorithm (BFGS)~\cite{BFGS} followed by the backbone to re-estimate the constants. 

==> main_content/preliminary_Wangyang.tex <==
\section{Background and Problem Statement}

\noindent\textbf{The Data to Equation ProblemFormal Definition.} 
The data to equation problem is 
Given an observation set $\mathcal{D} = (\mathbf{X}, y)$, where $\mathbf{X}$ represents input observations and $y$ denotes corresponding labels, the goal of SR is to automatically discover an optimal mathematical expression $f$. This expression should describe the relationship between $\mathbf{X}$ and $y$ in an interpretable manner, without requiring a predefined model structure.

\noindent\textbf{Transformer-based SR Model.} A Transformer-based SR model is trained on a large dataset comprising multiple observation sets and corresponding mathematical expressions $\{(\mathcal{D}_1, f_1),..., (\mathcal{D}_n, f_n)\}$. These expressions $f$ are presented as token sequences using prefix notation as in~\cite{lample2019deep}. The model encodes the observations into an embedding space and generates the target expression in an autoregressive manner.

% replace this name when we get a clear definition in the introduction
\noindent\textbf{Our Research Problem.} We aim to improve transformer-based SR models by addressing two key objectives: 
1) Incorporating equation representations as an additional modality to enhance the model's representation capacity;
2) Performing gradient-based search in the embedding space to identify the optimal embedding point for generating accurate symbolic equations.
\ul{To achieve goal 1}, given a specific testing dataset $\mathcal{D} = (\mathbf{X}, y)$, we designed an exploration module that randomly samples different observation sets and generates corresponding mathematical expressions $\{(\mathbf{X}_1, y_1, \Tilde{f}_1, \Tilde{y}_1),..., (\mathbf{X}_n, y_n, \Tilde{f}_n, \Tilde{y}_n\})$, where $\mathbf{X}_i$ represents a row-wise subset of $\mathbf{X}$ (i.e., a subset of samples), $\Tilde{y}_i$ is the generate pseudo-labels by $\Tilde{y}_i = \Tilde{f}_i(\mathbf{X}_i)$, and $n$ is the number of subsets. By incorporating the equations as the input, we fine-tune the SR model backbone from~\cite{kamienny2022end}, denoted as:
\begin{equation}
    \Tilde{f}_i = \psi(\mathcal{N}(\mathbf{X}_i, \Tilde{y}_i) \circ \mathcal{S}(\Tilde{f}_i)),
\end{equation}
where $\mathcal{N}$ and $\psi$ are the numerical encoder and decoder from the pre-trained backbone respectively, $\mathcal{S}$ is the symbolic encoder implemented by a transformer, and $\circ$ is the fusion operation (e.g., attention). The numerical and symbolic encoders collectively construct an embedding space $\mathcal{E}$.
\ul{To achieve goal 2}, we defined an evaluation metric to quantify the accuracy between $\Tilde{y}_i$ and the ground truth $y_i$. Then we developed an evaluator to assess the accuracy for a given vector $E$ in the embedding space $\mathcal{E}$. The evaluator provides gradient signals to guide the optimization process in $\mathcal{E}$. This gradient-steered search enables the model to locate the optimal embedding point, thereby generating the optimal equations $f^*$. It can be formulated by:
\begin{equation}
    f^* = \arg\max_{E \in \mathcal{E}} \mathcal{I}(\psi(E)),
\end{equation}
where $E$ is an embedding vector calculated by the fine-tuned numerical encoder and symbolic encoder, $\psi$ is the fine-tuned decoder, and $\mathcal{I}$ is the function for calculating the fitting accuracy between the predicted results and the ground truth labels. 
